Order of Compression: A Systematic and Optimal Sequence to Combinationally Compress CNN

Model compression has gained significant popularity as a means to alleviate the computational and memory demands of machine learning models. Each compression technique leverages unique features to reduce the size of neural networks. Although intuitively combining different techniques may enhance compression effectiveness, we find that the order in which they are combined significantly influences performance. To identify the optimal sequence for compressing neural networks, we propose the Order of Compression, a systematic and optimal sequence to apply multiple compression techniques in the most effective order. We start by building the foundations of the orders between any two compression approaches and then demonstrate inserting additional compression between any two compressions will not break the order of the two compression approaches. Based on the foundations, an optimal order is obtained with topological sorting. Validated on image-based regression and classification networks across different datasets, our proposed Order of Compression significantly reduces computational costs by up to 859 times on ResNet34, with negligible accuracy loss (-0.09% for CIFAR10) compared to the baseline model. We believe our simple yet effective exploration of the order of compression will shed light on the practice of model compression.

==> checklist.tex <==
\clearpage
\section*{Checklist}
Unless specified otherwise, please answer “yes” to each question if the relevant information is described either in the paper itself or in a technical appendix with an explicit reference from the main paper. If you wish to explain an answer further, please do so in a section titled “Reproducibility Checklist” at the end of the technical appendix.

This paper:
\begin{itemize}
\item Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes)
\item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes)
\item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (yes)
\end{itemize}

Does this paper make theoretical contributions? (no)

If yes, please complete the list below.
\begin{itemize}
\item All assumptions and restrictions are stated clearly and formally.
\item All novel claims are stated formally (e.g., in theorem statements).
\item Proofs of all novel claims are included.
\item Proof sketches or intuitions are given for complex and/or novel results.
\item Appropriate citations to theoretical tools used are given.
\item All theoretical claims are demonstrated empirically to hold.
\item All experimental code used to eliminate or disprove claims is included.
\end{itemize}

Does this paper rely on one or more datasets? (yes)

If yes, please complete the list below.
\begin{itemize}
\item A motivation is given for why the experiments are conducted on the selected datasets (yes)
\item All novel datasets introduced in this paper are included in a data appendix. (NA)
\item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (NA)
\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes)
\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes)
\item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (NA)
\end{itemize}

Does this paper include computational experiments? (yes)

If yes, please complete the list below.
\begin{itemize}
\item Any code required for pre-processing data is included in the appendix. (yes).
\item All source code required for conducting and analyzing the experiments is included in a code appendix. (yes, in form of a zip file)
\item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes)
\item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes)
\item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes, randomness is not important in our experiments)
\item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes, Some details are added in the Technical Appendix.)
\item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes)
\item This paper states the number of algorithm runs used to compute each reported result. (yes, Some details are added in the Technical Appendix.)
\item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes)
\item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes)
\item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes, Listed in the Technical Appendix.)
\item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes, Listed in the Technical Appendix.)
\end{itemize}

==> related.tex <==
\section{Related Work}
\vspace{-2mm}
%\jie{move this to intro: the point is there are studies for this important problem, however, none is comprehensive, and also equally importantly it is hard to compare them head-to-head, since each work takes on different settings.} 
%\jie{Moved to Intro}
To support the neural network on lightweight computing platforms, several compression techniques have been proposed in recent years. These techniques utilize different perspectives, such as network architecture, neuron, and bit precision, to compress DNN with a minimal accuracy compromise \cite{mishra2020survey, neill2020overview}. 
Meanwhile, characterized by fixed computational graphs and parameters during the inference stage, dynamic compression exhibits the ability to adapt network structures or parameters to varying inputs at runtime \cite{han2021dynamic}.
In applying multiple compressions, \cite{qi2021learning} combine pruning and quantization to compress CNNs and achieve about 50\% reduction in FLOPs with only 0.15\% to 0.37\% accuracy drops. \cite{li2023predictive} combine the early exit with quantization on CNN, which not only avoids floating-point computation, but also reduces over 50\% reduction in OPs with 1\% - 3\% accuracy drops.
Zhao \cite{zhao2023deep} presents the Deep Hybrid Compression Network. It uses relaxed mixed-precision quantization, relaxed weight pruning, and knowledge distillation to overcome the limitations of uniform quantization. \cite{han2015deep} leverage 
pruning, trained quantization, and Huffman coding to reduce the network parameter storage and energy cost in executing the neural network.
Although diverse compression methods are used on CNNs, limited research explores their interactions and optimal sequencing. Motivated by the potential to significantly reduce computation and parameter costs, this study investigates the interplay among compression techniques and establishes an optimal sequence for CNN compression.
